Internally Hankel $k$-positive systems

The classes of externally Hankel $k$-positive LTI systems and autonomous $k$-positive systems have recently been defined, and their properties and applications began to be explored using the framework of total positivity and variation diminishing operators. In this work, these two system classes are subsumed under a new class of internally Hankel $k$-positive systems, which we define as state-space LTI systems with $k$-positive controllability and observability operators. We show that internal Hankel $k$-positivity is a natural extension of the celebrated property of internal positivity ($k=1$), and we derive tractable conditions for verifying the cases $k> 1$ in the form of internal positivity of the first $k$ compound systems. As these conditions define a new positive realization problem, we also discuss geometric conditions for when a minimal internally Hankel $k$-positive realization exists. Finally, we use our results to establish a new framework for bounding the number of over- and undershoots in the step response of general LTI systems.

==> sec_cont.tex <==
\section{Extensions}
\label{sec:cont}
In this section, we first discuss extensions of our results in discrete-time (DT) to continuous-time (CT)
systems. This is followed by analogous results for the Toeplitz operator, as well as by applications 
to impulse/step-response analysis.

\subsection{Continuous-Time Systems}
The tuple $(A,b,c)$ is a CT state-space realization if 
\begin{equation}\label{eq:SISO_ct}
\begin{aligned}
\dot{x}(t) &= Ax(t) + bu(t), \\
y(t) &= cx(t), 
\end{aligned} 
\end{equation}
with $A \in \mathbb{R}^{n\times n}$, $b, c^\transp \in \mathbb{R}^n$. Its impulse response is
\begin{equation} 
    g(t) = c e^{A t} b s(t)
\end{equation}
and the controllability and observability operators are given by
\begin{subequations}
    \label{eq:CT_operators}
	\begin{align}
	\label{eq:CT_controllability}
	\Conct{}(A,b) u &:= \int_{-\infty}^{0_-} e^{-A\tau}b u(\tau) d\tau\\
	(\Obsct{}(A,c) x_0)(t) &:= ce^{A t} x_0, \ 
	x_0 \in \mathds{R}^n,  
	\ t\geq 0.
	\end{align}
\end{subequations}
As for DT systems, we assume $g$ to be absolutely integrable and $u$ to be bounded.  
By defining the variation of a continuous-time signal $u: \mathds{R} \to \mathds{R}$ as
\begin{equation*}
    \label{eq:CT_var}
    \varict{u} := \sup_{\substack{n \in \mathds{Z}_{>0} \\ t_1<\dotsc<t_n}} \; \vari{[u(t_1),\dotsc,u(t_n)]}
\end{equation*}
we can define internal Hankel $\ovd{k}$ as follows:
\begin{defn}
    \label{def:CT_internal_hankel_ovd_k}
    A CT system $(A,b,c)$ is called \textit{CT internally Hankel $\ovd{k}$} if $e^{At}$, $\Conct{}(A,b)$, and $\Obsct{}(A,c)$ are 
    $\ovd{k}$ for all $t \geq 0$.
\end{defn}
We seek to characterize these systems through an internal $k$-positivity notion. We will do so by discretization
of \cref{eq:CT_operators}, which allows us to apply our DT results. To this end, consider for $h , j > 0$, 
the \emph{(Riemann sum) sampled controllability operator}
\begin{subequations}
\label{eq:discretized_ops}
\begin{equation}
    \label{eq:discretized_ctr}
    \begin{split}
    \Conct{j,h}(A,b) u &:= h 
    \sum_{i=-j}^{-1} e^{-A ih} b u(ih) \\
    & = 
    h e^{Ah} 
    \Con{j}(e^{Ah},b)
    \left(
    \begin{array}{c}
         u(-h)  \\
         u(-2h) \\
         \vdots \\
         u(-jh)
    \end{array}
    \right)
    \end{split}
\end{equation}
and the \emph{sampled observability operator}  
\begin{equation}
    \label{eq:discretized_obs}
    \begin{split}
    \left(
    \begin{array}{c}
         y(h)  \\
         y(2h) \\
         \vdots \\
         y(jh)
    \end{array}
    \right)
     &= \Obs{j}(e^{Ah},c) e^{Ah} x_0 \\
     &=: \Obsct{j,h}(A,c) x_0.
    \end{split}
\end{equation}
\end{subequations}
Notice that for each $u$ and $x_0$ with finite variation there exist sufficiently large $j$ and small $h$ such that $\vari{\Conct{}(A,b)u} = \vari{\Conct{j,h}(A,b) u}$ 
and $\vari{\Obsct{}(A,c) x_0} = \vari{\Obsct{j,h}(A,c) x_0}$. Thus \cref{prop:k_pos_mat_var} allows connecting the $\ovd{k-1}$ property of the CT
operators \cref{eq:CT_operators} to $k$-positivity of the matrices $\Conct{j,h}(A,b)$ and 
$\Obsct{j,h}(A,c)$, where we consider all $j \ge k$. Since, from \cref{lem:compound_mat},
$k$-positivity of those matrices follows from $k$-positivity of $e^{Ah}$, $\Con{j}(e^{Ah},b)$, 
and $\Obs{j}(e^{Ah},c)$, \cref{def:CT_internal_hankel_ovd_k} is equivalent to the following CT analogue of
\cref{def:internal_hankel_kpos_}.
\begin{defn}
    \label{def:internal_kpos_CT}
    A CT system $(A,b,c)$ is called \textit{CT internally Hankel $\tp{k}$} if for all $h\in \mathds{R}_{>0}$ the DT system $(e^{Ah}, b,c)$ is (DT) internally Hankel $\tp{k}$.  \label{def:CT_internal_kpos}
\end{defn}
CT internal Hankel $k$-positivity can thus be verified by \cref{thm:Hankel_kpos_equiv}. However, we do not want
to do this for all $h >0$. Next, we will discuss how to eliminate the variable $h>0$ from the above
characterization. A classical result in that direction states that $e^{Ah} \geq 0$ for all $h \geq 0$ if and
only if $A$ is Metzler (nonnegative off-diagonal entries) \cite{Farina2000,berman1979nonnegative}. In general,
the compound matrix of $e^{At}$ can be expressed in terms of the \emph{additive compound matrix} 
\cite{muldowney1990compound}
\[ 
    A^{[j]} := \log(\compound{\exp(A)}{j}) = \left . \frac{d}{dh}\compound{e^{Ah}}{j} \right|_{h=0} 
\]  
which satisfies 
\begin{equation}
    \compound{e^{Ah}}{j} = e^{A^{[j]}h}. \label{eq:add_comp_exp}
\end{equation}
In other words, $e^{At}$ is $k$-positive if and only if $A^{[j]}$ is Metzler for $1\leq j\leq k$. The next result will also allow us to remove $h>0$ from the conditions involving $\Con{j}(e^{Ah},b)$ and
$\Obs{j}(e^{Ah},c)$:
\begin{thm}\label{thm:CT_equiv}
Let $(A,b,c)$ be a CT system such that $e^{Ah}$ is $k$-positive for all $h \in \mathds{R}_{>0}$. 
Then, the following holds:
\begin{enumerate}[i.]
    \item $\compound{\Con{j}(A,b)}{j} \geq 0$ for $1\leq j \leq k$ if and only if $\compound{\Con{j}(e^{Ah},b)}{j} \geq 0$ for all $1 \leq j \leq k$ and all $h \in \mathds{R}_{>0}$.
    \item $\compound{\Obs{j}(A,c)}{j} \geq 0$ for $1\leq j \leq k$ if and only if $\compound{\Obs{j}(e^{Ah},c)}{j} \geq 0$ for all $1 \leq j \leq k$ and all $h \in \mathds{R}_{>0}$.
\end{enumerate}
\end{thm}
\begin{proof}
We only show the first item, as the second follows analogously. 

Let us begin by showing that $\rk(\Con{j}(A,b)) = \rk(\Con{j}(e^{Ah},b))$. To see this note that if $\rk(\Con{j}(A,b)) < j$, then all $A^{i}b \in \im{C^{j-1}(A,b)}$ for all $i \geq j-1$, where $\im{\cdot}$ denotes the \emph{image (range)} of a matrix, which is why also $e^{Ah}b = \sum_{i=0}^{\infty} \frac{(Ah)^i}{i!}b \in \im{C^{j-1}(A,b)}$ and all $h >0$. Consequently, $\rk(\Con{j}(e^{Ah},b)) < j$. Conversely, if $\rk(\Con{j}(e^{Ah},b)) < j$, then by suitable column additions also $\rk(\Con{j}(I-e^{Ah},b)\diag(1,h,\dots,h^{j-1})^{-1}) = \rk(\Con{j}(h^{-1}(I-e^{Ah}),b)) < j$, which, due to the lower semi-continuity of the rank \cite{hiriart2013variational}, proves in the limit $h \to 0$ that $\rk(\Con{j}(A,b)) < j$.

Hence, we can assume that $\rk(\Con{j}(A,b)) = \rk(\Con{j}(e^{Ah},b)) = j$ as otherwise $\compound{\Con{j}(A,b)}{j}=0$ and the claim holds trivially. Let $\compound{\Con{j}(A,b)}{j} \geq 0$ for $1\leq j \leq k$. Then, $\compound{(F(\sigma)\Con{j}(A,b))}{j} > 0$
for all $\sigma > 0$ by \cref{prop:stp_aux_matrix} (iii). Suitable column additions within $\Con{j}(A,b)$ yield
that this equivalent to $\compound{(F(\sigma)\Con{j}(I+hA,b))}{j} > 0$ for all $\sigma, \; h > 0$. 
Since $(I+hA)b$ can be approximated arbitrarily well by $e^{Ah}b$ for sufficiently small $h > 0$, 
the continuity of the determinant \cite{horn2012matrix} implies the equivalence to $\compound{(F(\sigma) 
\Con{j}((I+hA),b))}{j} > 0$ for all $\sigma> 0$ and all sufficiently small $h > 0$. Hence, our claim follows for
for sufficiently small $h>0$ by invoking \cref{prop:stp_aux_matrix} (iv).

Finally, since $e^{Ah^\ast}$ is full rank and $k$-positive for all $h^\ast > 0$ as well as $e^{Ah^\ast}\Con{j}(A,b) = \Con{j}(A,e^{Ah^\ast}b)$, it follows that $\compound{\Con{j}(A,e^{Ah}b)}{j} \geq 0$ and $\rk(\Con{j}(A,e^{Ah^\ast}b)) = \rk(\Con{j}(A,b))$. Therefore, the result above can be applied to $\compound{\Con{j}(A,e^{Ah}b)}{j} \geq 0$, showing that $\compound{\Con{j}(e^{Ah},b)}{j} \geq 0$ for all $h > 0$.




\end{proof}
In particular, since $e^{Ah}$ has only positive eigenvalues, it follows from \cref{thm:cont_k_pos,thm:CT_equiv} 
that \cref{thm:Hankel_kpos_equiv} remains true in CT: 
\begin{thm}\label{thm:Hankel_kpos_equiv_CT}
    For a CT realization $(A,b,c)$, the following are equivalent for $k \geq 1$:
    \begin{enumerate}[i.]
        \item $(A,b,c)$ is CT internally Hankel $\ovd{k-1}$. 
        \item $(A,b,c)$ is CT internally Hankel $\tp{k}$.
        \item For $1 \le j \le k$, the \emph{$j$-th CT compound system realization} 
            \begin{equation}
                \label{eq:CT_compound_real}
                (A^{[j]}, \compound{\Con{j}(A,b)}{j},\compound{\Obs{j}(A,c)}{j}).  
            \end{equation}
        is CT internally positive.
    \end{enumerate}
\end{thm}
Note that our defined compound system realizations are indeed the CT compound systems, whose external positivity can be used to verify CT (external) Hankel $k$-positivity. 







    

Finally, an analogue to \cref{thm:real_simple} can be obtained by substituting \cref{eq:A_cond} with the condition in the following lemma, which extends the corresponding result in \cite{ohta1984reachability}.
\begin{lem}
Let $A \in \Rnn$ and $P \in \mathds{R}^{n \times K}$. Then, $e^{At} P = Pe^{Nt}$ with $e^{Nt}$ $k$-positive for all $t\geq 0$ if and only if there exits a $\lambda > 0$ such that $(A+\lambda I_n) P = P (N+\lambda I_K)$ with $(N+\lambda I_K)^{[j]}$ nonnegative for all $1\leq j\leq k$. 
\end{lem}
\begin{proof}
We begin by remarking the following properties of the additive compound matrix \cite{muldowney1990compound}: let $X,Y \in \Rnn$ and $Z \in \mathds{R}^{n \times K}$
\begin{enumerate}
    \item $(X+Y)^{[j]} = X^{[j]} + Y^{[j]}$
    \item $\compound{(e^{Xt}Z)}{j} = e^{X^{[j]}t} \compound{Z}{j}$
\end{enumerate}

$\Leftarrow$: Let $(A+\lambda I_n) P = P (N+\lambda I_K)$ for some $\lambda > 0$ such that $(N+\lambda I_K)^{[j]}$ is nonnegative for all $1\leq j\leq k$. Then, for all $\frac{i}{t} \geq \lambda$ with $t \geq 0$ and $i \in \mathds{N}$, it holds that $(A+\frac{i}{t}  I_n) P = P (N+\frac{i}{t}  I_K)$ and consequently
\begin{align*}
  e^{At} P = \lim_{i \to \infty}
  \left( I_n+\frac{At}{i}\right)^i P = P \lim_{i \to \infty}   \left( I_K+\frac{Nt}{i}\right)^i= P e^{Nt}.
\end{align*}
Moreover, by the first propety above $N^{[j]}$ is Metzler, which by \cref{eq:add_comp_exp} implies that $e^{Nt}$ is $k$-positive for $t \geq 0$.

$\Rightarrow$: Let $e^{At} P = Pe^{Nt}$ with $k$-positive $e^{Nt}$ for all $t \geq 0$. Then, by definition of the additive compound matrix and the properties above, it holds that
\begin{align*}
   (A+\lambda I_n)^{[j]}\compound{P}{j} &=  (A^{[j]}+\lambda I_n^{[j]}) \compound{P}{j} \\ 
   &=\compound{P}{j} (N^{[j]} + \lambda I_K^{[j]}) = \compound{P}{j} (N+ \lambda I_K)^{[j]}
\end{align*}
for all $\lambda \geq 0$,  $1\leq j \leq k$, where $N^{[j]}$ is Metzler by \cref{eq:add_comp_exp}. Thus, by choosing $\lambda$ sufficiently large, we conclude that $(N+ \lambda I_K)^{[j]}$ is nonnegative for all $1\leq j \leq k$. 
\end{proof}

\subsection{Internal Toeplitz $k$-positivity}
Next, we want to see whether there also exists a 
meaningful internal counterpart to the property of external
\emph{Toeplitz} $k$-positivity from  \cite{grussler2020variation}.
The \emph{Toeplitz operator} of a DT system $G(z)$ is defined as
\begin{equation*}
(\Toep{g} u)(t) = \sum_{\tau=0}^{t} g(t-\tau)u(\tau),
\ t \geq 0. \label{eq:def_toep_disc} 
\end{equation*}
Similarly to the Hankel case, external Toeplitz $\ovd{k-1}$ and
$k$-positivity can be characterized based on the
Toeplitz matrix \cite{grussler2020variation}:
\small{
\begin{equation*}%
T_g(t,j) := \begin{pmatrix}
g(t) & g(t-1) & \dots & g(t-j+1)\\
g(t+1) & g(t) & \dots & g(t-j)\\
\vdots & \vdots & \ddots   & \vdots \\
g(t+j-1)   & g(t+j-2) & \dots & g(t)\\
\end{pmatrix}
\end{equation*}}
\normalsize
Unfortunately, unlike the Hankel operator, the Toeplitz operator lacks an 
interpretable decomposition in terms of state-space operators, so
that defining an internal version of Toeplitz $k$-positivity becomes
less natural and somewhat ambiguous.

Next, we outline one possibility of defining internal Toeplitz $\ovd{k}$. To this end, consider the system $(A,b,c)$ with \emph{state transition map} 
\[
    x(t) = (\Flow{}(A,b)[x_0,u])(t) := A^t x_0 +  
    \sum_{\tau=0}^{t-1} A^{t-\tau-1} b u(\tau), \ t\geq 0
\]
and \emph{output transition map}
\[
    y(t) = (\mathcal{G}(A,b,c)[x_0,u])(t) := c(\Flow{}(A,b)[x_0,u])(t), 
    \ t\geq 0.
\]
Note that $\Flow{}$ and $\mathcal{G}$ act on the sequence 
$(x_0^\transp,u(0),u(1),\dotsc)$, that is, $x_0$ is stacked in front of
$u_{[0,\infty]}$. We then define the Toeplitz counterpart to the internal
$\ovd{k}$ property as follows.
\begin{defn}
	\label{def:internal_toeplitz_kpos} 
	$(A,b,c)$ is called \emph{internally Toeplitz 
	$\ovd{k}$} if $\Flow{}(A,b)$ and $\mathcal{G}(A,b,c)$  
	are $\ovd{k}$. 
\end{defn}
Thus internal Toeplitz $\ovd{k}$ requires a system to be $\ovd{k}$ from 
$(x_0^\transp,u_{[0,\infty]})$ to the state $x(t)$ and output $y$. Note
that if $u =0$, then $(\Flow{}[x_0,0])(t) = A^t x_0$ and $\mathcal{G}(A,b,c)[x_0,0])(t) = (\Obs{}(A,c) x_0)(t)$, requiring $A$ and $\Obs{t}(A,c)$ to be $\ovd{k}$ for all $t \in \mathds{Z}_{>0}$. Further, if $x_0 = 0$, then $(\Flow{}[0,u])(t) = \rCon{t}(A,b) u_{[0:t-1]}$, where
\[
    \rCon{t}(A,b) = \begin{pmatrix}
    A^{t-1}b & \dots & b
    \end{pmatrix}, \; \rCon{0}(A,b) := ( \; )
\]
implying that also $\rCon{t}(A,b)$ is $\ovd{k}$ for all $t \in \mathds{Z}_{>0}$. For $k=0$, this means that the internal Toeplitz and Hankel $\ovd{0}$ correspond to internal positivity. In general, however, the reversing the column order in $\Con{t}(A,b)$ yields different system properties, as known from the external case \cite{grussler2020variation}. 
Our internal Toeplitz notion further requires that $\mathcal{X}^t := 
\begin{pmatrix} A^t & \rCon{t-1}(A,b) \end{pmatrix}$ and
\begin{equation*}
    \mathcal{Y}^t :=
    \begin{pmatrix}
    \Obs{t}(A,b) & T_g(0,t-1)
    \end{pmatrix}
\end{equation*}
to be $\ovd{k}$ for all $t \in \mathds{Z}_{>0}$.

While, similarly to \cref{thm:cont_k_pos}, this may be checked with a finite
number of conditions for $\mathcal{X}^t$, it is much less clear how this can be done for $\mathcal{Y}^t$. Finally, there is no compound system
interpretation that naturally extends the notion of internal positive
realization.

\subsection{Impulse and step response analysis}
Tracking of the over- and undershooting behaviour of a step response is a classical problem in control that resembles (see e.g. \cite{aastrom2010feedback}) the trade-off between fast rise and settling times. For LTI systems, the total number of over- and undershoots equals the number of sign changes in the impulse response. While there are several lower bounds \cite{swaroop1996some,damm2014zero,elkhoury1993influence,elkhoury1993discrete}, there only exist few upper bounds \cite{elkhoury1993influence,elkhoury1993discrete}. Next, we will see that our analysis builds the foundation for a framework of upper bounds. 

The impulse response of a system $G(z)$ with realization $(A,b,c)$ equals $g(t) = (\Obs{}(A,c)b)(t)$. 
Therefore, if $\Obs{}(A,c)$ is $k$-positive, then the impulse response of $(A,b,c)$ changes its sign at 
most $\vari{b}$ times for all $\vari{b} \leq k-1$, and has the same sign-changing order as $b$ in case
of equality. 

Similarly to \cref{thm:real_simple}, we conclude the following result:
\begin{thm} \label{cor:impulse}
Let $(A,b,c)$ be an observable realization of $G(z)$. Then, there exists a realization $(A_+,b_+,c_+)$ of $G(z)$ such that $A_+$ and $\Obs{}(A_+,c_+)$ are $k$-positive if and only if there exists a $P \in \mathds{R}^{n \times K}$, $K \geq n$ such that $AP = PA_+$ and $\compound{\Obs{j}(A,c)}{j}^\transp \in \cone(\compound{P}{j})^\ast$, $1 \leq j 
\leq k$. 
\end{thm}
\begin{proof}
$\Rightarrow$: Follows as in the proof to \cref{thm:real_simple}. 

$\Leftarrow$: Let $A$ and $\Obs{}(A_+,c_+)$ be $k$-positive. Then by the Kalman observability decomposition, there exists a transformation $T = \begin{pmatrix} P \\ \ast  \end{pmatrix}$ such that
\begin{align*}
T A_+ = \begin{pmatrix} 
A & 0\\
\ast & \ast
\end{pmatrix} T, \quad c_+ = \begin{pmatrix} c & 0 \end{pmatrix} T.
\end{align*}
Consequently, $AP = PA_+$, $c_+ = cP$ and therefore $\compound{\Obs{j}(A,c)}{j} \compound{P}{j} = \compound{\Obs{j}(A_+,c_+)}{j}$.
\end{proof}

Since the realization $(A_+,b_+,c_+)$ may not be unique, it remains an open question how to minimize the
sign changes in $b_+$ in order to make the upper bound the least conservative. We will leave an
answer to this question to future work. It should be noted that the approach in \cite{elkhoury1993discrete} essentially corresponds to the case where a realization with a totally positive observability operator exits, because it assumes positive distinct real poles and real zeros, apart from multiple poles at zero. To simplify the treatment of multiple poles at zero, we remark the following corollary that applies to all $A$ in Jordan form $\sigma(A) \subset \mathds{R}_{\geq 0}$. 
\begin{cor}\label{cor:poles_origin}
Let $(A,c)$ be such that $\compound{\Obs{j}(A,c)}{j} \geq 0$ for all $1\leq j \leq k$ and $\rk(\Obs{j}(A,c)) = j$ for all $1 \leq j\leq k-1$. Further, assume there exists an $\varepsilon > 0$ such that $A+\eta I$ is $k$-positive for all $\eta \in [0,\varepsilon]$. Then, $\Obs{}(A,c)$ is $k$-positive. 
\end{cor}
\begin{proof}
Since $\Obs{j}(A+\eta I,c)$ results from column addition in $\Obs{j}(A,c)$, it follows that 
$\compound{\Obs{j}(A,c)}{j} \geq 0$ if and only if $\compound{\Obs{j}(A+\eta I,c)}{j} \geq 0$ and 
$\rk(\Obs{j}(A,c)) = \rk(\Obs{j}(A+\eta I,c))$. However, $\rk(A+\eta I)$ is full and therefore it 
suffices to check the rank condition on $\Obs{j}(A+\eta I,c)$ in order to conclude from
\cref{thm:cont_k_pos} that $\Obs{}(A+\eta I,c)$ is $k$-positive. By continuity of the minors (see~e.g. 
\cite{horn2012matrix}), it follows then that also $\Obs{}(A,c)$ is $k$-positive.
\end{proof}

